Real-Time, Deep Synthetic Aperture Sonar (SAS) Autofocus

Synthetic aperture sonar (SAS) requires precise time-of-flight measurements of the transmitted/received waveform to produce well-focused imagery. It is not uncommon for errors in these measurements to be present resulting in image defocusing. To overcome this, an \emph{autofocus} algorithm is employed as a post-processing step after image reconstruction to improve image focus. A particular class of these algorithms can be framed as a sharpness/contrast metric-based optimization. To improve convergence, a hand-crafted weighting function to remove "bad" areas of the image is sometimes applied to the image-under-test before the optimization procedure. Additionally, dozens of iterations are necessary for convergence which is a large compute burden for low size, weight, and power (SWaP) systems. We propose a deep learning technique to overcome these limitations and implicitly learn the weighting function in a data-driven manner. Our proposed method, which we call Deep Autofocus, uses features from the single-look-complex (SLC) to estimate the phase correction which is applied in $k$-space. Furthermore, we train our algorithm on batches of training imagery so that during deployment, only a single iteration of our method is sufficient to autofocus. We show results demonstrating the robustness of our technique by comparing our results to four commonly used image sharpness metrics. Our results demonstrate Deep Autofocus can produce imagery perceptually better than common iterative techniques but at a lower computational cost. We conclude that Deep Autofocus can provide a more favorable cost-quality trade-off than alternatives with significant potential of future research.

==> reviewer_responses/reviewer2.tex <==
1. It is recommended to add some details of the deep autofocus network. For example, how to process the DRC image and phase image by the Densenet121 network? What is the network architecture of the Dense module?

Thank you for attention to detail.  We elaborated in the manuscript on the DRC function, how the DRC and phase are input to the Densenet121, the contents of the Densenet121 network, and the description of the Dense module. 

2. I argue that the autofocus algorithm proposed by the authors does not differ much from traditional methods in principle, such as using the image sharpness metric as an optimization goal, such as estimating phase error parameters using regression methods. Therefore, can the authors theoretically analyze the advantages of the proposed method over traditional methods? For example, the algorithm needs iterative training to obtain error estimates, but why is the computation time two orders of magnitude lower than traditional methods?

Thank you for your comment.  Our method is fundamentally different than any phase array autofocus method we have seen previously. A recent overview paper of Deep Learning for SAS TODO paper also confirms this. Upon reading the last question, we think there is a simple misunderstanding of the method by the reviewer.  The answer to your last question is that our deep network does not run iteratively at inference time (the time when you autofocus an image).  The iterations are only needed for analyzing defocused images to have the network learn features and a phase correction to improve the image focus.  In practice, the network is trained on a small training set of SLC's collected from the SAS.  Once trained, the network is deployed on a SAS system to autofocus imagery in real-time as it comes out of the beamformer -- no training data or iterations are necessary during this time as you feed the image under test to the network and it (in a single forward pass) outputs the autofocused image.  The benefit of not having to run an iterative optimization procedure for each image is one of the benefits of our method.

==> reviewer_responses/reviewer3.tex <==

The manuscript, entitled “Deep Autofocus for Synthetic Aperture Sonar”, studies a post-processing step to improve image quality for synthetic aperture sonar (SAS). A deep learning image processing scheme is introduced in this manuscript and some experimental results verify the validity of the post-processing step for SAS. The manuscript is easy to follow and the idea is straightforward. However, I cannot recommend acceptance of this manuscript for the following reasons:
1)      The deep learning method itself is not novel. It is obvious that this manuscript only introduces a deep learning image processing method for SAS. Although it may be true that this is the first try to apply deep learning for SAS, it is still unacceptable. The authors should emphasize their efforts on improving deep learning image processing methods for their application. Of course, deep learning is a powerful tool, it can be applied anywhere. When considering that it only applies to the reconstructed image as a post-processing step, it is the same as image processing with deep learning methods, and thus it is not novel.

Thank you for your comment and for reviewing our work. We further reviewed the literature on synthetic aperture processing and were unable to substantiate your claim of "it is the same as image processing with deep learning methods" as we could not find any methods for image processing for image focus improvement that operated in $k$-space and required only a single forward pass to compute the autofocused output image. We welcome the reviewer to provide us with a reference as acknowledge we could have missed it.

2)      It is uncommon that the number of images for training is much less than that for validation and test, where only 120 images is used for training. Although data augmentation is used in this manuscript, the overfitting problem may still occur.

Obtaining SAS data is quite expensive so little imagery is often available for training (for example, we are only aware of one complex-valued SAS datasets publicly available).  Additionally, deep learning methods often work well but only when abundant training data is available.  To demonstrate the robustness of our proposed method, we opted to use a small test set as this it demonstrates that our method can produce good results even when little training data is present, and it represents training data sizes not uncommonly seen in practice.

3)      The benchmark and the proposed deep autofocus are run in two different platforms, their mean runtimes cannot be compared in this case, and it is totally unfair.

The comparison the manusript makes is between runtimes of the gradient descent-based methods (which are commonly used in practice) and our proposed method.  There is roughly two orders of magnitude improvement in run-time for our method versus the comparison methods. All of these methods were run on the same GPU.  You are correct in that the benchmark method was run on a different platform (i.e. a CPU).  However, we do not suggest in the manuscript that this run-time should be compared to our method as a benefit in any way.  We provided this time in the table to highlight the rigor we provided in creating our benchmark dataset in the absence of available ground truth completely focused imagery.  We state in the manuscript that this type of imagery is impossible to come by except in simulation as there is often residual phase error present in a real SAS image which cannot be detected by human inspection. Therefore, we run a sophisticated optimizer to try to autofocus the images as best as possible approaching the results a simulation would give; the runtime of the benchmark is listed to highlight this sophistication. We had to forgo using simulated results for two reasons: One, a publicly available SAS simulation providing realistic seafloor texture does not exist. Two, writing such a simulator is quite expensive to construct.

4)      From the figures provided by the authors, the performance can only be improved marginally.

Thank you for your comment.  We show in Table TODO that our run-timer performance is improved by two orders of magntitude over the traditional methods while our average image quality is at least as good as traditional methods.  Furthermore, for all the image quality comparisons, we show that our proposed method provides a much higher lower bound of image degradation for difficult cases.  This can be seen by examining the left tail of each quiver plot in Figure 5 and observe that the Deep Autofocus has a better worse case than all of the comparison methods.  TODO we have updated the manuscript to make this more clear.
